Tight Polynomial Bounds for Loop Programs in Polynomial Space

We consider the following problem: given a program, find tight asymptotic bounds on the values of some variables at the end of the computation (or at any given program point) in terms of its input values. We focus on the case of polynomially-bounded variables, and on a weak programming language for which we have recently shown that tight bounds for polynomially-bounded variables are computable. These bounds are sets of multivariate polynomials. While their computability has been settled, the complexity of this program-analysis problem remained open. In this paper, we show the problem to be PSPACE-complete. The main contribution is a new, space-efficient analysis algorithm. This algorithm is obtained in a few steps. First, we develop an algorithm for univariate bounds, a sub-problem which is already PSPACE-hard. Then, a decision procedure for multivariate bounds is achieved by reducing this problem to the univariate case; this reduction is orthogonal to the solution of the univariate problem and uses observations on the geometry of a set of vectors that represent multivariate bounds. Finally, we transform the univariate-bound algorithm to produce multivariate bounds.

==> fig-multipath.tex <==
\begin{figure}[t]
% Had the last instruction been changed to $\X_3 \pass \X_3 + \X_2$, the value of $3@3$ would fail to be uniquely defined, but the code would also
% produce exponential growth when iterated.}{t}{fig-multipath}
\[\xymatrix@R=20pt{
& \X_3 \pass \X_2+\X_3 & \X_2 \pass \X_1*\X_3 &  \X_3 \pass \X_1+\X_2 & \X_2 \pass \X_1 \\
  x_1\ar@{->}[r] & x_1 \ar@{->}[r]  \ar@{->}[dr]  & x_1  \ar@{->}[r] \ar@{->}[ddr]  & x_1  \ar@{->}[dr] \ar@{->}[r]& x_1\\
  x_2 \ar@{->}[r]\ar@{->}[dr]  & x_2 & x_2^{\fbox{\tiny 3\char64 2}}\ar@{->}[dr] \ar@{->}[r] & x_2 & x_2 \\
  x_3^{\fbox{\tiny 3\char64 0}}\ar@{->}[r] & x_3^{\fbox{\tiny 3\char64 1}}\ar@{->}[ur]\ar@{->}[r]   & x_3  & x_3^{\fbox{\tiny 3\char64 3}}\ar@{->}[r] & x_3^{\fbox{\tiny 3\char64 4}}
%   x_4\ar@{->}[r] & x_4\ar@{->}[r]   & x_4  & x_4\ar@{->}[r] & x_3
}\]
\caption{An illustration for Lemma~\ref{lem:i@t}, showing the data-flow along a sequence of four instructions, presumably forming a path through a loop's body.
The annotations highlight the path whereby the value $x_3$ of variable ${\tt X}_3$ at time 0 flows until it ends up in ${\tt X}_3$ again at time 4.
If such a path exists, it is unique.}\label{fig-multipath}
\end{figure}


==> maxdegree.tex <==
\section{Bounding the Attainable Degree}%
\label{sec:degree}

The purpose of this section is to prove a bound on the maximal attainable degree in terms of the program size.
Specifically, we consider the computation of program $P$ (i.e., any core-language command)
on an initial state ${\vec x} = \tuple{x_1,x_2,\dots,x_n}$.
 We restrict attention to polynomially-bounded programs\footnote{Inspecting the proof shows that the requirement here is that any part of $P$ is polynomially bounded, in other words, this applies
 to intermediate results as well, and not only to final values.
However, the method we described in Section~\ref{sec:outline} for excluding exponentially-growing
 variables achieves exactly that.
}, so that the bound
on the final value of any chosen variable can be given as a set of monomials
(all monomials are worst-case lower bounds and their \textbf{max} is a tight upper bound).
Our goal is to bound the degrees of these monomials by a function of, roughly, the
size of $P$.    The proof is based on the analysis $\sempar{C}^M$ as given in Section~\ref{sec:ev-multivariate}.
First, we introduce the \emph{dependence graph} for a loop, which will be used in the proof.

In Section~\ref{sec:proof} we introduced the Dependence Graph of a multi-polynomial, denoted $G({\vec p})$.
In the following proof we associate a graph with a command $\C$ used as a loop body.  This graph is the union of
$G({\vec p})$ over all ${\vec p} \in \closure{\sempar{C}^S}$, or, alternatively, ${\vec p} \in \closure{\sempar{C}^M}$ (the reader is invited
to check that these two definitions coincide, due to the correctness of the analyses).   We denote this graph
by $G(\C)$.

\begin{lem}\label{lem:qacyclic-G}
Suppose that $\C$ is the body of a polynomially-bounded loop. Then: (1) $G(\C)$ is transitively closed;
(2) If $i,j$ belong to a cycle in $G({\C})$, then in any ${\vec p} \in \sempar{C}^M$, ${\vec p}[i]$ may include $x_j$ only if
${\vec p}[i] = x_j$.
\end{lem}

\begin{proof}
(1) follows easily from the definitions, because the graph is based on the closure set.  If $G$ has arc $i\to j$ due to some ${\vec p}\in\closure{\sempar{C}^M}$,
and arc $j\to k$ due to some ${\vec q}\in\closure{\sempar{C}^M}$, then it has $i\to k$ due to ${\vec q}\acirc {\vec p}$ which is also in the closure.

For (2), we first note that by the closure property, it such a cycle exists then there are also direct arcs $i\to j\to i$.
Suppose, by contradiction, that ${\vec p}[i] = x_j  m$ for some non-trivial monomial $m$ (i.e., not 1 or 0).    Since
there is also an arc $i\to j$, there is ${\vec q}\in \closure{\sempar{C}^M}$ such that
$x_i | {\vec q}[j] $ ($x_i$ divides the non-zero monomial ${\vec q}[j]$).
Then we have
\[ x_j m \mathrel{|} ({\vec q}\acirc {\vec p})[j] \,. \]
By the soundness of the analysis, $({\vec q}\acirc {\vec p})[j]$ is an attainable lower bound on the worst-case result of  a finite sequence of loop iterations;
in concrete terms, it means that given initial concrete (numeric) state $\vec x  = \tuple{x_1,\dots,x_n}$, after executing that finite sequence of iterations, we can have
$x'_j \ge d (x_j m(\vec x))$, for a constant $d>0$; as $m$ is an increasing function of the variables on which it depends, it means that for sufficiently large
initial values, we have $x'_j \ge 2x_j$, and iterating the same sequence
generates exponential growth, contradicting the assumption of polynomial boundedness.
\end{proof}

Note that as the graph is transitively closed, it consists of a set of SCCs (strongly connected components) which are complete subgraphs, and reducing every SCC to a single node
we get the acyclic \emph{component graph}. If a variable is never modified in the loop, it's SCC will be a singleton and have no predecessor in the component graph.

To support the PSPACE complexity classification, we want to relate the maximum attainable degree to the \emph{size} of program $P$ --- not a precisely defined
measure since we have not given a concrete syntax to our language~---~but in fact, we will relate it to the measure defined next, which would be lower than or,
at most, polynomially related
to any reasonable measure of size.  As will be seen in the proof, what we are trying to measure is really the length of certain chains of data-flow in the program,
along which the degree of the bounds can possibly grow.

\newcommand{\ipl}[1]{{\Vert \pgt{#1} \Vert}}
\newcommand{\maxdeg}[0]{\mathop{\mathrm{maxdeg}}}

\begin{defi}
For a Core-Language command \C, we define $\ipl{C}$ as follows.
\begin{alignat*}{3}
&\ipl{\amul{i}{j}{k}} &&= 1 , \\
&\ipl{C} &&= 0 &&\text{if \C\ is any other assignment or \pgt{skip}}, \\
&\ipl{\pgt{choose C or D}} && = \max(\ipl{C},\ipl{D}) , \\
&\ipl{C;D} && = \ipl{C}+\ipl{D} ,\\
&\ipl{\pgt{loop X}\ \{\C\}} && = n^2 \ipl{C} \,.
\end{alignat*}
\end{defi}

Another simple definition and we are ready for the main result of this section.

\begin{defi}
For a monomial $m(\vec x) = {\vec x}^{\vec d}$, let $\deg(m) = \sum_i d_i$.
For an AMP $\vec p$,
$\maxdeg(\vec p)$ be the highest value of $\deg(m)$ where $m$ ranges on all monomials in $\vec p$.
 For a command {\C}, let
$\maxdeg(\C)$ be the highest value of $\maxdeg({\vec p})$ where ${\vec p}$ ranges on all AMPs in $\sempar{C}^M$.
\end{defi}

\begin{thm}
For any polynomially-bounded command \C, $\maxdeg(\C) \le 2^{\ipl{C}}$.
\end{thm}

\begin{proof}
The proof is by structural induction. The multiplication command can square a variable, and therefore has a $\maxdeg$ of $2 = 2^1$.

All other assignment commands as well as \pgt{skip} do not generate any non-linear monomial and so have a $\maxdeg$ of $1 = 2^0$.

The induction step for \pgt{choose} is obvious.

For \pgt{C;D}, we note that $\deg(m\acirc {\vec p}) \le \deg(m)\cdot \maxdeg({\vec p})$ (this can be reached, e.g., $m=x_1x_2$ and
${\vec p} = \tuple{x_1^3, x_1^3}$);
so by induction we have
\[  \maxdeg(\pgt{C;D}) \le \maxdeg(\D)\cdot \maxdeg(\C) \le 2^{\ipl{C} + \ipl{D}} = 2^{\ipl{C;D}} \,.\]

Finally for loops we need inner inductions, given as the next set of lemmas, which yield (Lemma~\ref{lem:deg-of-loop}) the conclusion
\[\maxdeg \sempar{\pgt{loop X}\ \{\C\}}^M \le 2^{n^2 \ipl{C}} = 2^{\ipl{\pgt{loop X}\ \{\C\}}} .\]
\end{proof}

Assume {\C} to be the body of a polynomially-bounded loop. Based on Lemma~\ref{lem:qacyclic-G},
we can assume (w.l.o.g.) that the program's variables are (re-)indexed, for the scope of an argument concerning this particular loop, so that the
order of the indices agrees with the topological order of the component graph of $G({\C})$; this means that in any ${\vec p}\in \sempar{C}^M$,
${\vec p}[i]$ can depend only on $x_1,\dots,x_i$. In fact, it depends only on $x_1,\dots,x_{i-1}$ unless it is precisely $x_i$ (Lemma~\ref{lem:qacyclic-G}).
Also, w.l.o.g., we may assume that the loop bound is $x_1$ (since it must
be a variable which is not modified throughout the loop).

\begin{lem}\label{lem:deg-of-Cl}
Assume {\C} to be the body of a polynomially-bounded loop, with the above assumptions regarding indices.
Also assume that {\C} is known to satisfy $\maxdeg(\C) \le 2^{\ipl{C}}$.
Let ${\vec p} \in \closure{\sempar{C}^M}$.
Then for any $i$, $\deg {\vec p}[i] \le 2^{(i-1)\ipl{C}}$.
\end{lem}

\begin{proof}
The proof is by induction on the steps in the construction of $\vec p$, according to the equation
\[ \closure{\setS} = \{ \idppol \} \, \cup\,  \setS \acirc \closure{\setS} \,. \]
The base-case is ${\vec p} = \idppol$, where the lemma clearly holds.

In the induction step, we assume
$\vec r$ to satisfy the lemma and let ${\vec p} = {\vec q}\acirc {\vec r}$ with ${\vec q}\in \sempar{C}^M$.
We want to bound the degree of ${\vec p}[i]$.  Now, if ${\vec q}[i] = x_i$, the result follows because it's assumed to hold for $\vec r$.
Otherwise, by assumption, $\deg {\vec q}[i] \le 2^{\ipl{C}}$. By the assumption on the indices, all variables appearing in ${\vec q}[i]$ are
among $x_1,\dots,x_{i-1}$ and by assumption, the degree of ${\vec r}[j]$ for $j\le i-1$ is bounded by $2^{(i-2)\ipl{C}}$.
Now
\[ \deg {\vec p}[i] \le \deg {\vec q}[i] \cdot \max(\deg {\vec r}[1],\dots,\deg {\vec r}[i-1]) \le 2^{(i-1)\ipl{C}} \,. \]
\end{proof}

\begin{lem}
Assume {\C} to be the body of a polynomially-bounded loop, with the above assumptions regarding indices.
Also assume that {\C} is known to satisfy $\maxdeg(\C) \le 2^{\ipl{C}}$.
Let ${\vec p} \in Gen(1,\closure{\sempar{C}^M})$.
Then for any $i$, $\deg {\vec p}[i] \le 2^{(n\ipl{C}}$.
\end{lem}

\begin{proof}
Generalization can increase the degree of a monomial by at most 1 (multiplying it by the loop variable, $x_1$ under our assumptions).
So, based on the previous lemma, the bound stated is not only true but, in fact, exaggerated (just to get a simple formula).
\end{proof}

\begin{lem}\label{lem:deg-of-loop}
Assume {\C} to be the body of a polynomially-bounded loop, with the above assumptions regarding indices.
Also assume that {\C} is known to satisfy $\maxdeg(\C) \le 2^{\ipl{C}}$.
Let ${\vec p} \in \closure{Gen(1,\closure{\sempar{C}^M})}$.
Then for any $i$, $\deg {\vec p}[i] \le 2^{((i-1)n\ipl{C}}$.
\end{lem}

\begin{proof}
The proof is the same as for Lemma~\ref{lem:deg-of-Cl}, using the last lemma for a bound on $\vec q$ in the composition ${\vec q}\acirc {\vec r}$.
\end{proof}

Clearly the above bounds are all below $ 2^{n^2 \ipl{C}} $, as required for completing the proof of our main result.


==> removed-example.tex <==
\begin{exa}\label{ex:md-reduction}
Consider the following loop.
\begin{Verbatim}[codes={\catcode`$=3\catcode`_=8}]
loop X$_5$ {
  choose
    choose { X$_3$ := X$_1$; X$_4$ := X$_2$ } or { X$_3$ := X$_2$; X$_4$ := X$_1$ }
   or
      X$_1$ := X$_3$ + X$_4$
}
\end{Verbatim}
One possible execution simulates two iterations, specifically the first branch (two assignments) followed by the last one, and making a selection
so that $M_{11}=\eps$ and $M_{21}=1$. This  results in the addition of the instruction
$\amul{1}{2}{5}$. Another execution path simulates the following four iterations:
\begin{Verbatim}[codes={\catcode`$=3\catcode`_=8}]
      X$_1$ := X$_3$ + X$_4$;
      X$_3$ := X$_1$; X$_4$ := X$_2$;
      X$_1$ := X$_3$ + X$_4$;
      X$_3$ := X$_1$; X$_4$ := X$_2$;
\end{Verbatim}
and makes choices so that, at the end, $M_{33}=\eps$ and $M_{23}=1$; hence it
adds $\amul{3}{2}{5}$. The reader may verify that another execution adds $\amul{4}{2}{5}$.  Thus the final transformed program is the following
(for readability we flex the syntax and use a choice command with multiple branches).
\begin{Verbatim}[codes={\catcode`$=3\catcode`_=8}]
loop X$_5$ {
  choose
     choose { X$_3$ := X$_1$; X$_4$ := X$_2$ } or { X$_3$ := X$_2$; X$_4$ := X$_1$ }
   or
      choose   X$_1$ := X$_3$  or  X$_1$ := X$_4$
    or
      choose  X$_1$ := X$_2$*X$_5$  or  X$_3$ := X$_2$*X$_5$  or  X$_4$ := X$_2$*X$_5$
}
\end{Verbatim}

\end{exa}

